Investigating End-Users' Values in Agriculture Mobile Applications Development: An Empirical Study on Bangladeshi Female Farmers

The omnipresent nature of mobile applications (apps) in all aspects of daily lives raises the necessity of reflecting end-users values (e.g., fairness, honesty, etc.) in apps. However, there are limited considerations of end-users values in apps development. Value violations by apps have been reported in the media and are responsible for end-users dissatisfaction and negative socio-economic consequences. Value violations may bring more severe and lasting problems for marginalized and vulnerable end-users of apps, which have been explored less (if at all) in the software engineering community. However, understanding the values of the end-users of apps is the essential first step towards values-based apps development. This research aims to fill this gap by investigating the human values of Bangladeshi female farmers as a marginalized and vulnerable group of end-users of Bangladeshi agriculture apps. We conducted an empirical study that collected and analyzed data from a survey with 193 Bangladeshi female farmers to explore the underlying factor structure of the values of Bangladeshi female farmers and the significance of demographics on their values. The results identified three underlying factors of Bangladeshi female farmers. The first factor comprises of five values: benevolence, security, conformity, universalism, and tradition. The second factor consists of two values: self-direction and stimulation. The third factor includes three values: power, achievement, and hedonism. We also identified strong influences of demographics on some of the values of Bangladeshi female farmers. For example, area has significant impacts on three values: hedonism, achievement, and tradition. Similarly, there are also strong influences of household income on power and security.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


